Freezing of Gait Detection Using Gramian Angular Fields and Federated Learning from Wearable Sensors

Freezing of gait (FOG) is a debilitating symptom of Parkinson's disease that impairs mobility and safety by increasing the risk of falls. An effective FOG detection system must be accurate, real-time, and deployable in free-living environments to enable timely interventions. However, existing detection methods face challenges due to (1) intra- and inter-patient variability, (2) subject-specific training, (3) using multiple sensors in FOG dominant locations (e.g., ankles) leading to high failure points, (4) centralized, non-adaptive learning frameworks that sacrifice patient privacy and prevent collaborative model refinement across populations and disease progression, and (5) most systems are tested in controlled settings, limiting their real-world applicability for continuous in-home monitoring. Addressing these gaps, we present FOGSense, a real-world deployable FOG detection system designed for uncontrolled, free-living conditions using only a single sensor. FOGSense uses Gramian Angular Field (GAF) transformations and privacy-preserving federated deep learning to capture temporal and spatial gait patterns missed by traditional methods with a low false positive rate. We evaluated our system using a public Parkinson's dataset collected in a free-living environment. FOGSense improves accuracy by 10.4% over a single-axis accelerometer, reduces failure points compared to multi-sensor systems, and demonstrates robustness to missing values. The federated architecture allows personalized model adaptation and efficient smartphone synchronization during off-peak hours, making it effective for long-term monitoring as symptoms evolve. Overall, FOGSense achieved a 22.2% improvement in F1-score and a 74.53% reduction in false positive rate compared to state-of-the-art methods, along with enhanced sensitivity for FOG episode detection.

==> tables/cnn_branch_arch_table.tex <==
\begin{table}[!h]
   \centering
   \begin{tabular}{lcccc}
   \toprule
   \textbf{Layer} & \textbf{Filters} & \textbf{Kernel} & \textbf{Regularization} & \textbf{Dropout} \\ 
   \midrule
   Conv2D-1 & 32 & 3×3 & None & 20\% \\
   BatchNorm & - & - & - & - \\
   MaxPool2D & - & 2×2 & - & - \\
   \midrule
   Conv2D-2 & 64 & 3×3 & L2 ($\lambda=0.001$) & 20\% \\
   BatchNorm & - & - & - & - \\
   MaxPool2D & - & 2×2 & - & - \\
   \midrule
   Conv2D-3 & 128 & 3×3 & L2 ($\lambda=0.001$) & 40\% \\
   BatchNorm & - & - & - & - \\
   MaxPool2D & - & 2×2 & - & - \\
   \bottomrule
   \end{tabular}
   \vspace{2pt}
   \caption{Architecture of Each CNN Branch}
   \label{tab:cnn_branch_architecture}
   \vspace{-25pt}
\end{table}

==> tables/concise_cnn_branch_arch.tex <==
\begin{table}[!h]
    \centering
    \label{tab:cnn_branch_architecture}
    \begin{tabular}{lccc}
    \toprule
    \textbf{Layer} & \textbf{Filters} & \textbf{Regularization} & \textbf{Dropout} \\ \midrule
    First  & 32 & None & 20\% \\ 
    Second & 64 & L2 ($\lambda=0.001$) & 20\% \\ 
    Third  & 128 & L2 ($\lambda=0.001$) & 40\% \\ \bottomrule
    \end{tabular}
    \vspace{2pt}
    \caption{Architecture of Each CNN Branch}
    \vspace{-20pt}
\end{table}

==> tables/first_table.tex <==

% First table
\begin{table}[h!]
\centering
\begin{tabular}{|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
\hline
\textbf{No of Channels} & \textbf{Channel Configuration} & \textbf{Total Training Time} & \textbf{Total Test Time} & \textbf{Epochs} \\
\hline
3 & (AccAP, AccML, AccV) & 3780 s & 12.88 s & 60 \\

2 & (AccAP, AccML) & 1924.42 s & 15.39 s & 60 \\

2 & (AccML, AccV) & 1908.48 s & 18.95 s & 60 \\

2 & (AccAP, AccV) & 1904.34 s & 13.31 s & 60 \\

1 & (AccAP) & 3882.32 s & - & 60 \\

1 & (AccML) & 2271.88 s & - & 60 \\

1 & (AccV) & 3659.41 s & - & 60 \\

\hline
\end{tabular}
\caption{Training and Testing Time for Different Channel Configurations}
\label{tab:part1}
\end{table}

==> tables/second_table.tex <==

% Second table
\begin{table}[h!]
\centering
\begin{tabular}{|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
\hline
\textbf{Channel Configuration} & \textbf{Accura-cy} & \textbf{F1 Score (Avg)} & \textbf{Sensiti-vity} & \textbf{Preci-sion} \\
\hline
(AccAP, AccML, AccV) & 87.23\% & 90.31\% & 91.03\% & 90.27\% \\

(AccAP, AccML) & 93.24\% & 87.67\% & 93.24\% & 93.24\% \\

(AccML, AccV) & 95.30\% & 90.75\% & 95.29\% & 95.29\% \\

(AccAP, AccV) & 94.45\% & 90.49\% & 94.45\% & 94.45\% \\

(AccAP) & 93.25\% & 78.98\% & 93.25\% & 93.25\% \\

(AccML) & 94.98\% & 83.71\% & 96.16\% & 96.16\% \\

(AccV) & 95.00\% & 73.27\% & 95.00\% & 95.00\% \\
\hline
\end{tabular}
\caption{Performance Metrics for Different Channel Configurations}
\label{tab:part2}
\end{table}

==> tables/table2.tex <==
\begin{table}[!h]
\begin{minipage}{\linewidth}
\resizebox{\linewidth}{!}{%
   \centering
   \begin{tabular}{
       @{}
       C{1cm}
       C{3cm}
       S[table-format=2.2,table-alignment=center]
       S[table-format=2.2,table-alignment=center]
       S[table-format=2.2,table-alignment=center]
       S[table-format=2.2,table-alignment=center]
       S[table-format=2.2,table-alignment=center]
       c
       @{}
   }
   \toprule
   \thead{\centering Channels} & 
   \thead{\centering Input Combination} & 
   {\thead{\centering Train Time (s/epoch)}} & 
   {\thead{\centering Test Time (s)}} & 
   {\thead{\centering Accuracy (\%)}} & 
   {\thead{\centering F1 Avg (\%)}} & 
   {\thead{\centering Precision (\%)}} \\
   \midrule
   \multirow{1}{*}{\centering 3} & 
   AccAP-AccML-AccV & {--} & {--} & {--} & {--} & {--} \\
   \midrule
   \multirow{3}{*}{\centering 2} & 
   AccAP-AccML & 32.87 & 20.88 & 90.70 & 82.84 & 90.70 \\
   & AccML-AccV & 31.38 & 14.45 & 93.29 & 93.17 & 93.29 \\
   & AccAP-AccV & 31.11 & 20.85 & 89.33 & 74.29 & 89.33 \\
   \midrule
   \multirow{3}{*}{\centering 1} &
   AccAP & {--} & {--} & {--} & {--} & {--} \\
   & AccML & {--} & {--} & {--} & {--} & {--} \\
   & AccV & {--} & {--} & {--} & {--} & {--} \\
   \bottomrule
   \end{tabular}
   }
   \end{minipage}
   \vspace{5pt}
   
   \small
   \caption{With Mixmatch in Validation}
   \label{tab:with-mixmatch}
\end{table}
